XHand: Real-time Expressive Hand Avatar

Hand avatars play a pivotal role in a wide array of digital interfaces, enhancing user immersion and facilitating natural interaction within virtual environments. While previous studies have focused on photo-realistic hand rendering, little attention has been paid to reconstruct the hand geometry with fine details, which is essential to rendering quality. In the realms of extended reality and gaming, on-the-fly rendering becomes imperative. To this end, we introduce an expressive hand avatar, named XHand, that is designed to comprehensively generate hand shape, appearance, and deformations in real-time. To obtain fine-grained hand meshes, we make use of three feature embedding modules to predict hand deformation displacements, albedo, and linear blending skinning weights, respectively. To achieve photo-realistic hand rendering on fine-grained meshes, our method employs a mesh-based neural renderer by leveraging mesh topological consistency and latent codes from embedding modules. During training, a part-aware Laplace smoothing strategy is proposed by incorporating the distinct levels of regularization to effectively maintain the necessary details and eliminate the undesired artifacts. The experimental evaluations on InterHand2.6M and DeepHandMesh datasets demonstrate the efficacy of XHand, which is able to recover high-fidelity geometry and texture for hand animations across diverse poses in real-time. To reproduce our results, we will make the full implementation publicly available at https://github.com/agnJason/XHand.

==> sec/3_method.tex <==
\section{Method}

\begin{figure*}[tb]
    \centering
    \includegraphics[width=1.0 \linewidth]{figs/overview.pdf}
    \caption{\textbf{Overview of XHand}. Given a hand pose $\theta$, XHand utilizes three feature embedding modules to obtain the displacement field $D$, Linear Blending Skinning (LBS) weights $W$, and albedos $\rho$. These features are applied to the subdivided MANO template $\bar{\mathcal{M}}'$, resulting in a detailed geometric hand mesh. Leveraging mesh-based neural rendering, we achieve photo-realistic renderings. XHand can generate both detailed geometry and realistic rendering in real-time.} 
    \label{fig:overview}
    \vspace{-0.20in}
\end{figure*}

Given multi-view images $\{I_{t,i}|i=1,...,N,t=1,...,T\}$ for $T$ frames captured from $N$ viewpoints with pose $\theta$ and shape $\beta$ of their corresponding MANO~\cite{MANO} parametric hand models $\{\mathcal{M}(\theta_t, \beta)|t = 1,...,T\}$, our method aims to recover expressive personalized hand meshes with skin wrinkles and render photo-realistic image in real-time. An overview of our method is shown in Fig.~\ref{fig:overview}. Given the hand pose parameters $\theta$, the fine-grained mesh is obtained from feature embedding modules (Sec.~\ref{sec:fe}), in which are designed to obtain LBS weights, vertex displacements and albedos by combining the average features of the mesh with pose-driven feature mapping. Therefore, detailed hands under different poses are generated by driving and refining the template mesh. With the fine-grained posed mesh, the mesh-based neural renderer achieves real-time photo-realistic rendering based on the vertex albedos $\rho$, normals $\mathcal{N}$, and latent code $Q$ in feature embedding modules.
%In this section, we initially describe the parametric hand model required to build XHand in Sec.~\ref{sec:mano}, the hand avatar representation in Sec.~\ref{sec:xhand}, and the explanation for how our model can be effectively trained in Sec.~\ref{sec:training}.
%Our approach employs a combination of multiple embeddings. Linear Blending Skinning (LBS) weights are derived from the LBS Embedding $E_{lbs}$, while the Displacement Embedding $E_{D}$ generates displacements for hand skin, additionally, the Albedo Embedding $E_{\rho}$ is utilized to obtain the mesh albedo.

\subsection{Feature Embedding Module}
\label{sec:fe}

%XAvatar~\cite{xavatar} employs a point-sampling approach to train each neural field, which is computationally intensive. In contrast, 
%To simplify the learning objective, we propose an effective feature embedding module to handle various poses. 
It is challenging to learn the distinctive features of hands in different poses. To better separate between the deformation caused by changes in posture and the inherent characteristics of the hand, we propose an efficient feature embedding module that relies on average features of hand mesh and computes offsets of features in different poses, as presented in Fig.~\ref{fig:emb}. 

By providing a personalized hand mesh $\mathcal{M}$ and hand pose $\theta_t$ at a certain time $t$, our feature embedding module generates mesh features $f_\mathcal{M}$ as follows \begin{equation}
    f_\mathcal{M} = E(\theta_t | \bar{f}_\mathcal{M}),
\end{equation} $\bar{f}_\mathcal{M}$ denotes the average features of the hand mesh. 
%It is challenging for MLPs to discern the influence of specific conditions on mesh features, which may lead to divergence in results. \textbf{WHY?} 
To represent the mesh features of personalized hand generated under the influence of hand poses, we design the following embedding function
\begin{equation}
    E(\theta_t | \bar{f}_\mathcal{M}) = \bar{f}_\mathcal{M} + e(\theta_t, Q) * \mathcal{K},
\end{equation} where $Q$ is vertex latent code to encode different vertices and $e$ denotes a pose decoder, which is combined with multi-layer perceptrons (MLPs), used to project the pose $\theta_t$ and latent code $Q$ into the implicit space. To align with the feature space, $\mathcal{K}$ is the mapping code to convert implicit space $\mathbb{R}^{m}$ onto feature space $\mathbb{R}^{n}$, which satisfies $\sum_{j=1}^{n} \mathcal{K}_{ij} = 1, \quad \text{for } i = 1, 2, \ldots, m$. %The pipeline of the feature embedding is presented in Fig.~\ref{fig:emb}.

\begin{figure}[tb]
	\centering
        \includegraphics[width=0.7\textwidth]{figs/embeding.pdf}
	\caption{\textbf{Our proposed feature embedding module}. Given pose $\theta$ at time $t$, $\theta_t$ is decoded by pose decode $e$ along with vertex latent features $Q$ and mapped to the feature space through mapping code $\mathcal{K}$. Finally, it is combined with the average vertex feature $\bar{f}_\mathcal{M}$ to obtain the feature for the pose $\theta$. We introduce three different feature embedding modules $E_{lbs}$, $E_{D}$ and $E_{\rho}$ to predict LBS weights $W'$, displacements $D$ and albedos $\rho$. }
	\label{fig:emb}
    \vspace{-0.20in}
\end{figure}

The separation of personalized hand mesh and poses allows for the interpretable acquisition of hand features $f_\mathcal{M}$ corresponding to the pose $\theta_t$. Moreover, with the constraint of average features $\bar{f}_\mathcal{M}$, the feature embedding demonstrates faster convergence and improves accuracy. Our approach employs a combination of multiple embeddings. Linear Blending Skinning (LBS) weights are derived from the LBS embedding $E_{lbs}$, while the displacement embedding $E_{D}$ generates displacements for vertex positions, additionally, the albedo embedding $E_{\rho}$ is utilized to obtain the mesh albedos. The three feature embedding modules $E_{lbs}$, $E_{D}$ and $E_{\rho}$ with their corresponding latent code $Q_{lbs}$, $Q_D$ and $Q_\rho$ make use of the same structure of $E(\theta_t | \bar{f}_\mathcal{M})$ except that the target features $f$ are different.



\subsection{XHand Model}
\label{sec:xhand}
There are various alternatives available for hand avatar representation~\cite{bib:handavatar,handnerf, bib:LISA, livehand, xavatar}, while simultaneously achieving real-time generation of detailed geometry and realistic rendering poses a significant challenge.
To tackle the intricate hand skin variations and achieve photo-realistic hand rendering, we propose a hand avatar model XHand by taking advantage of mesh-based neural representation. %Specifically, our model has three distinct feature embedding modules: 1) $E_D$ accounts for the geometry through an implicit displacement field; 2) $E_{lbs}$ takes consideration of deformation using learned forward LBS with continuous skinning weights; 3) $E_{\rho}$ treats appearance as an albedo value. %These feature embeddings present the intricate details of hand geometry, deformation, and appearance so as to achieve highly fidelity hand avatars.

% {\bf FUSE THE FOLLOWING TEXT INTO SECTION 2. JUST NEED A SINGLE SENTENCE TO ADDRESS MOTIVATION OF HAND AVATAR. There are various alternatives available for hand avatar representation, such as HandAvatar~\cite{bib:handavatar}, HandNeRF~\cite{handnerf}, LiveHand~\cite{livehand}, or XAvatar~\cite{xavatar}. NeRF-based methods~\cite{handnerf, livehand} offer guaranteed neural rendering with lack of the ability to generate realistic meshes. HandAvatar~\cite{bib:handavatar} offers both rendering and reconstruction capabilities, while the results tend to be relatively smooth. XAvatar~\cite{xavatar} provides animatable characters while introducing complexity in computations due to its sampling method. }


We leverage the parametric hand model MANO~\cite{MANO} as the initialisation of hand geometry. It effectively maps the pose parameter $\theta \in \mathbb{R}^{J\times3}$ with $J$ per-bone parts and the shape parameter $\beta \in \mathbb{R}^{10}$ onto a template mesh $\bar{\mathcal{M}}$ with $V$ vertices. Such mapping is achieved by utilizing linear blend skinning with the weights $W \in \mathbb{R}^{V\times J}$, which is defined as follows 
\begin{equation}
    \mathcal{M} = MANO(\bar{\mathcal{M}}, W, \theta, \beta),
\end{equation}
where $\mathcal{M}$ is the posed hand mesh.
%\noindent\textbf{Mesh Subdivision.} To increase mesh resolution and expressive capacity, we perform a uniform subdivision of the MANO template mesh $\bar{\mathcal{M}}$ by introducing new vertices at the midpoints of existing edges. Therefore, we can obtain a high resolution template mesh $\bar{\mathcal{M}}'$ with 49,281 vertices and 98,432 faces. Subsequently, the LBS weights of new vertices are assigned as the average of the seminal vertices.

\noindent\textbf{Geometry Refinement.} After increasing the MANO mesh resolution for fine geometry using the method in~\cite{bib:handavatar}, a personalized vertex displacement field $D$ is introduced to allow extra deformation for each vertex of the template mesh. The refined posed hand mesh $\mathcal{M}_{fine}$ can be obtained by
\begin{equation}
    \bar{\mathcal{M}}', W' = \mathcal{S}(\bar{\mathcal{M}}, W), \end{equation} \begin{equation} \label{eq:mesh}
    \mathcal{M}_{fine} = MANO(\bar{\mathcal{M}}' + D, W', \theta, \beta),
\end{equation} where $\mathcal{S}$ is the subdivision function for mesh. To enhance the fidelity of the skin geometry, the vertex displacement $D$ is pose-dependent for each individual, enabling an accurate representation of the deformation under different poses. 

To better represent the intricate details of hand mesh and improve the precision of the manipulation, three feature embedding modules $E_{\rho}$, $E_{D}$ and $E_{lbs}$ are employed. Given hand pose parameters $\{\theta_{t}|t=1,...,T\}$ for $T$ frames, we predict features of the mesh as follows \begin{equation}
    \rho_t = E_{\rho}(\theta_t),D_t = E_D(\theta_t),W'_t = E_{lbs}(\theta_t),
\end{equation} where $\rho_t$ represents the vertex albedo, $D_t$ denotes displacement, and $W'_t$ is LBS weight under $t$ pose. The refined mesh $\mathcal{M}_{fine}$ at time $t$ can be formulated as below
\begin{equation}
    \mathcal{M}_{fine} = MANO(\bar{\mathcal{M}}' + D_t, W'_t, \theta_t, \beta).
\end{equation}


\noindent\textbf{Inverse Rendering.} In order to train the three feature embedding modules $E_{\rho}$, $E_D$ and $E_{lbs}$ simultaneously, an inverse renderer is employed to render hand images. Assuming that the skin color follows the Lambertian reflectance model~\cite{sfs}, the renderer $B$ can be calculated by the Spherical Harmonics coefficients $\mathbf{G}$, the vertex normal $\mathcal{N}$, and the vertex albedo $\rho$ using the following equation \begin{equation}\label{eq:render}
    B(\pi^i) = \rho\cdot SH(\mathbf{G}, \mathcal{N}),
\end{equation} where $\pi^i$ is camera parameter of $i$-th viewpoint. $SH(\cdot)$ represents Sphere Harmonic (SH) function of the third order. $\mathcal{N}$ is the vertex normal computed from the vertices of mesh $\mathcal{M}_{fine}$. The application of inverse rendering along with the Lambertian reflectance model effectively disentangles geometry and appearance by analyzing how the variations in brightness across surface relate to its underlying shape.
%Therefore, we can effectively utilize the geometric and albedo of the mesh to achieve rapid and differentiable rendering.

\noindent\textbf{Mesh-based Neural Rendering.}
The NeRF-based methods usually employ volumetric rendering along its corresponding camera ray $\mathbf{d}$ to acquire pixel color~\cite{handnerf,livehand} while they require a large amount of training time. Instead, to minimize sampling time and decrease computation, we employ a mesh-based neural rendering method to obtain photo-realistic image by taking advantage of the preserved topology of our refined mesh. % This method leverages the preserved topology of our refined hand representation, resulting in enhanced visual fidelity. 

The mesh is explicitly represented by triangular facets so that the intersection points between rays and meshes are located within the facets. The features that describe meshes, such as position, color, and normal, are associated with their respective vertices. Consequently, the attributes of intersection points are calculated by interpolating the three vertices of triangular facet to its intersection point. The efficient differentiable rasterization~\cite{Laine2020diffrast} ensures the feasibility of inverse rendering and mesh-based neural rendering.

Given a camera view $\pi^i$, our proposed mesh-based neural rendering $\mathcal{C}(\pi^i)$ is calculated with position $\mathbf{x}$, normal $\mathcal{N}$, feature vector $\mathbf{h}$ and ray direction $\mathbf{d}$ \begin{equation}
    \mathcal{C}(\pi^i) = c(\mathbf{x}, \mathcal{N}, \mathbf{h}, \mathbf{d}),
\end{equation} 
where $\mathbf{x}$, $\mathbf{h}$ and $\mathcal{N}$ are obtained through interpolation with $\mathcal{M}_{fine}$. $\mathbf{h}$ contains latent codes $Q_D$ and $Q_\rho$ detached from $E_D$ and $E_\rho$, and rendering latent codes $Q_{render}$. The neural renderer $\mathcal{C}$ is parameterized with an 8-layer MLP. % We introduce a rendering network~\cite{chan2022efficient} that can re-render the output through pixel-aligned features in a 3D consistent manner. 

\subsection{Training Process}
\label{sec:training}

To get a personalized hand representation, the parameters of the three feature embedding modules $E_D$, $E_{lbs}$, and $E_{\rho}$, as well as the neural renderer $\mathcal{C}$, require to be optimized using multi-view image sequences. Our training process consists of three steps, including initialization, training of feature embedding modules, and training of the mesh-based neural renderer.

\noindent\textbf{Initialization of XHand.}
To train XHand, the average features $\bar{f}_\mathcal{M}$ of mesh in feature embedding significantly affect training efficiency and results. Random initialization has great impact on training due to estimation errors in $E_{lbs}$ and $E_D$, which may lead to the failure of inverse rendering. Therefore, it is crucial to initialize the neural hand representation. To this end, the reconstruction result of the first frame ($t=1$) is served as the initial model. 

Inspired by~\cite{bib:nccsfs,gan2024}, XHand model is initialized from multi-view images. The vertex displacement $D$ and vertex albedo $\rho$ of hand mesh are jointly optimized through inverse rendering. Mesh generation is obtained from Eq.~\ref{eq:mesh}, and the rendering equation is same with Eq.~\ref{eq:render}. The loss function during initialization is formulated as below \begin{equation}\begin{aligned}
    \mathcal{L}_{init} = \sum\limits_{i}||B(\pi^i) - I_i||_1 + \sum L * D + \sum L * \rho,
\end{aligned}\end{equation} where $L$ is the Laplacian matrix~\cite{nealen2006laplacian}. Laplacian smoothing terms $L * D$ and $L * \rho$ are employed to constrain the optimization, given that the mesh features are supposed to be smooth. The outcomes $D$ and $\rho$ are used to initialize $E_D$ and $E_\rho$. The initialization of $E_{lbs}$ is directly derived from MANO~\cite{MANO}.

\noindent\textbf{Loss Functions of Feature Embedding.}
Inverse rendering is utilized to learn the parameters of three feature embedding modules $E_D$, $E_{lbs}$ and $E_{\rho}$. $\mathcal{L}_{inv}$ is introduced to minimize the errors of rendering images as follows\begin{equation}
    \mathcal{L}_{inv} = \mathcal{L}_{rgb} + \mathcal{L}_{reg},
\end{equation} where $\mathcal{L}_{rgb}$ represents the rendering loss. $\mathcal{L}_{reg}$ is the regularization term. In terms of $\mathcal{L}_{rgb}$, inspired by Kerbl~\textit{et al.}~\cite{kerbl20233d}, we use $L_1$ error combined with a SSIM term as below \begin{equation} \begin{aligned} \label{eq:rgb}
    \mathcal{L}_{rgb} &= \lambda\sum\limits_{i}||B(\pi^i) - I_i||_1 + (1-\lambda)\mathcal{L}_{SSIM}(B(\pi^i), I_i),
\end{aligned}\end{equation} where $\lambda$ denotes trade-off coefficient. %$\mathcal{L}_{inv}$ is used to minimize the loss of inverse rendering, optimizing the parameters of feature embeddings. $\mathcal{L}_{neu}$ minimizes the error of mesh-based neural rendering.%, while the latent code of the feature embeddings is detached, preventing the gradient from propagating forward.

To enhance the efficiency of extracting geometric information from images, the part-aware Laplace smoothing $\mathcal{L}_{pLap}$ is introduced. The Laplace matrix $\mathbf{A}$ of mesh feature $f$ is defined as $\mathbf{A} = L * f$. Hierarchical weights $\phi_{pLap}$ are introduced to balance the weights of regularisation via different levels of smoothness. $\varphi_{i}$ in matrix $\phi_{pLap}$ is defined as follows \begin{equation}
\varphi_{i} = \left\{\begin{array}{l} \gamma_{1} \quad 0 < \mathbf{A}_{i} < p_1 
\\ \gamma_{2} \quad p_1 < \mathbf{A}_{i} < p_2
\\ ...
\end{array}\right.
,
\end{equation} where $p$ represents the threshold values for the hierarchical weighting and $\gamma$ denotes the balanced coefficient. The part-aware Laplace smoothing $\mathcal{L}_{pLap}$ is used to reduce excessive roughness in albedo and displacement without affecting the fine details, defined as follows \begin{equation}
    \mathcal{L}_{pLap}(f) = \sum\limits_{i} \phi_{pLap}\mathbf{A}.
\end{equation} By employing varying degrees of hierarchical weights to trade-off Laplacian smoothing, $\mathcal{L}_{pLap}$ is able to better constrain feature optimization in different scenarios. In our cases, minor irregularities are considered acceptable, while excessive changes are undesirable. Therefore, the threshold $p$ can be dynamically controlled through the quantiles of Laplace matrix $A$, where those greater than $p$ will be assigned larger balance coefficients.%, such as restricting significant variations while allowing minor changes.

The following regularization terms are introduced to conform the optimized mesh to the shape of the hand
\begin{equation} \begin{aligned}
\mathcal{L}_{reg} &= \mathcal{L}_{pLap}(\rho) + \mathcal{L}_{pLap}(D) \\ & + \alpha_{1}\mathcal{L}_{mask} + \alpha_{2}\mathcal{L}_{e} + \alpha_{3}\mathcal{L}_{d}.\label{eq:eq1}
\end{aligned}\end{equation} $\mathcal{L}_{pLap}(\rho)$ and $\mathcal{L}_{pLap}(D)$ are part-aware Laplacian smoothing terms to maintain albedos and displacement flattening during training. $\mathcal{L}_{mask}$, $\mathcal{L}_{e}$ and $\mathcal{L}_{d}$ are utilized to ensure that the optimized hand mesh remains close to the MANO model, where each term is assigned with constant coefficients denoted by $\alpha_1, \alpha_2$ and $\alpha_3$. $\mathcal{L}_{mask}$ represents the $L_1$ loss between the mask $\hat{M}$ rendered during inverse rendering and the original MANO mask $M$\begin{equation}
    \mathcal{L}_{mask} = \sum\limits_{i}||\hat{M} - M||_1.
\end{equation} $\mathcal{L}_{e}$ penalizes the edge length changes of $E_{ij}$  with respect to MANO mesh
\begin{equation} \mathcal{L}_{e} = \sum\limits_{i,j}||\hat{E_{ij}} - E_{ij}||_2^2,\end{equation} 
 where $\hat{E_{ij}}$ is obtained by calculating the Euclidean distance $||\cdot||_2^2$ between adjacent vertices $V_i$ and $V_j$ on the mesh edges. $E_{ij}$ denotes the edge distance of the subdivided MANO mesh $\bar{\mathcal{M}}'$. 
$\mathcal{L}_{d}$ is employed to constrain the degree of displacement caculated by the Euclidean distance as below \begin{equation} \mathcal{L}_{d} = \sum\limits_{i}||D_i||_2^2.\end{equation} 

\noindent\textbf{Loss Functions of Neural Renderer.}
Once the latent codes $Q_D$ and $Q_\rho$ of $E_D$ and $E_\rho$ are detached, $\mathcal{L}_{neu}$ is presented to minimize the residuals between the rendered image and the ground truth like Eq.~\ref{eq:rgb}\begin{equation*} %\begin{aligned}
    \mathcal{L}_{neu} = \omega\sum\limits_{i}||\mathcal{C}(\pi^i) - I_i||_1 + (1-\omega)\mathcal{L}_{SSIM}(\mathcal{C}(\pi^i), I_i),
%\end{aligned}
\end{equation*}
where $\omega$ denotes balanced coefficient.

==> sec/3_method_old.tex <==
\section{Method}

\begin{figure*}
    \centering
    \includegraphics[width=1 \linewidth]{figs/overview.pdf}
    \vspace{-0.15in}
    \caption{\textbf{Overview of XHand.}. Given a hand pose $\theta$, XHand utilizes three well-designed feature embeddings modules to obtain the displacement field $D$, Linear Blending Skinning (LBS) weights $W$, and albedo $\rho$. These features are applied to the subdivided MANO template $\bar{\mathcal{M}}'$, resulting in a detailed geometric hand mesh. Leveraging mesh-based neural rendering, we achieve photo-realistic renderings. XHand can generate both detailed geometry and realistic rendering in real-time.} 
    \label{fig:overview}
    \vspace{-0.15in}
\end{figure*}

Given multi-view images $\{I_{tj}|i=1...N,t=1...T\}$ for $T$ frames captured from $N$ viewpoints and their corresponding MANO~\cite{MANO} parametric hand models $\{\mathcal{M}(\theta_t, \beta)|t = 1...T\}$ with pose $\theta$ and shape $\beta$, our method creates expressive hand meshes and photo-realistic renderings that can accurately reflect hand-pose and skin wrinkles in real-time. An overview of our method is shown in Fig.~\ref{fig:overview}. Given the hand pose parameters $\theta$, the fine-grained mesh is obtained from our presented feature embeddings scheme, in which $E_{lbs}$, $E_{D}$ and $E_{\rho}$ are meticulously designed to obtain LBS weights, displacements and albedo by combining the average features of the mesh with pose-driven feature mapping. Thus, detailed hands under different $\theta$ poses are generated by driving and refining the template mesh.
Given extrinsic and intrinsic camera parameters, the mesh-based neural renderer achieves real-time photo-realistic rendering based on the mesh vertex albedo $\rho$, normals $\mathcal{N}$, and latent code $Q_D$ and $Q_\rho$ in feature embedding $E_{D}$ and $E_{\rho}$.
%In this section, we initially describe the parametric hand model required to build XHand in Sec.~\ref{sec:mano}, the hand avatar representation in Sec.~\ref{sec:xhand}, and the explanation for how our model can be effectively trained in Sec.~\ref{sec:training}.
%Our approach employs a combination of multiple embeddings. Linear Blending Skinning (LBS) weights are derived from the LBS Embedding $E_{lbs}$, while the Displacement Embedding $E_{D}$ generates displacements for hand skin, additionally, the Albedo Embedding $E_{\rho}$ is utilized to obtain the mesh albedo.

\subsection{MANO-based Model}
\label{sec:mano}

We leverage the parametric hand model MANO~\cite{MANO} as the foundation of initial hand geometry. It effectively maps the pose parameter $\theta \in \mathbb{R}^{J\times3}$ with $J$ per-bone parts and the shape parameter $\beta \in \mathbb{R}^{10}$ into a posed mesh $\mathcal{M}$. Such mapping is achieved by enforcing the LBS weights $W \in \mathbb{R}^{V\times B}$ to a template hand mesh $\bar{\mathcal{M}}$ with $V$ vertices, which is defined as follows 
\begin{equation}
    \mathcal{M}(\theta, \beta) = MANO(\bar{\mathcal{M}}, W, \theta, \beta).
\end{equation}

\noindent\textbf{Mesh Subdivision.} To increase mesh resolution and expressive capacity, we perform a uniform subdivision o the MANO template mesh $\bar{\mathcal{M}}$ by introducing new vertices at the midpoints of existing edges. Therefore, we can obtain a high resolution template mesh $\bar{\mathcal{M}}'$ with 49,281 vertices and 98,432 faces. Subsequently, the LBS weights of new vertices are assigned as the average of the seminal vertices.

\noindent\textbf{Geometry Refinement.} By leveraging the increased mesh resolution for fine geometry details, a person-specific vertex displacement field $D$ is introduced to allow extra deformation for each vertex in the template mesh. The posed hand mesh could be obtained by
\begin{equation}
    \bar{\mathcal{M}}', W' = \mathcal{S}(\bar{\mathcal{M}}, W), \end{equation} \begin{equation} \label{eq:mesh}
    \mathcal{M}_{fine}(\theta, \beta) = MANO(\bar{\mathcal{M}}' + D, W', \theta, \beta),
\end{equation} where $\mathcal{S}$ is the subdivision function for mesh. To enhance the fidelity of the skin geometry, the vertex displacement $D$ is pose-dependent for each individual. %, enabling an accurate representation of the deformation under different poses. 


\subsection{XHand Model}
\label{sec:xhand}

There are various alternatives available for hand avatar representation~\cite{bib:handavatar,handnerf, bib:LISA, livehand, xavatar}, while simultaneously achieving real-time generation of detailed geometry and realistic rendering poses a significant challenge.
To tackle the intricate hand skin variations and achieve photo-realistic hand rendering, we propose a hand avatar model XHand by taking advantage of mesh-based neural representation. Specifically, our model has three distinct feature embeddings: 1) $E_D$ accounts for the geometry through an implicit displacement field; 2) $E_{lbs}$ takes consideration of deformation using learned forward LBS with continuous skinning weights; 3) $E_{\rho}$ treats appearance as an albedo value. These feature embeddings present the intricate details of hand geometry, deformation, and appearance so as to achieve highly fidelity hand avatars.% {\bf FUSE THE FOLLOWING TEXT INTO SECTION 2. JUST NEED A SINGLE SENTENCE TO ADDRESS MOTIVATION OF HAND AVATAR. There are various alternatives available for hand avatar representation, such as HandAvatar~\cite{bib:handavatar}, HandNeRF~\cite{handnerf}, LiveHand~\cite{livehand}, or XAvatar~\cite{xavatar}. NeRF-based methods~\cite{handnerf, livehand} offer guaranteed neural rendering with lack of the ability to generate realistic meshes. HandAvatar~\cite{bib:handavatar} offers both rendering and reconstruction capabilities, while the results tend to be relatively smooth. XAvatar~\cite{xavatar} provides animatable characters while introducing complexity in computations due to its sampling method. }

Given hand pose parameters $\{\theta_{t}|t=1...T\}$ for $T$ frames, we predict features of the mesh as follows \begin{equation}
    \rho_t = E_{\rho}(\theta_t),D_t = E_D(\theta_t),W'_t = E_{lbs}(\theta_t),
\end{equation} where $\rho_t$ represents the vertex albedo. $D_t$ denotes displacement, and $W'_t$ is LBS weight under $t$ pose. The refined mesh $\mathcal{M}^t_{fine}$ at moment $t$ can be formulated as below
\begin{equation}
    \mathcal{M}^t_{fine} = MANO(\bar{\mathcal{M}}' + D_t, W'_t, \theta_t, \beta).
\end{equation}

\begin{figure}
	\centering
        \includegraphics[width=0.45\textwidth]{figs/embeding.pdf}
        \vspace{-0.1in}
	\caption{\textbf{Our proposed feature embedding module.} Given event $p$ at moment $t$, $p$ is decoded by Event Decode $e$ along with vertex latent features $Q$ and mapped to the feature space through Mapping Code $\mathcal{K}$. Finally, it is combined with the average vertex feature $\bar{f}_\mathcal{M}$ to obtain the feature for the event $p$.}
	\label{fig:emb}
	\vspace{-0.2in}
\end{figure}

\noindent\textbf{Feature Embedding.} 

%XAvatar~\cite{xavatar} employs a point-sampling approach to train each neural field, which is computationally intensive. In contrast, 
Instead of using a computationally intensive point-sampling approach to train each neural field like~\cite{xavatar}, we propose an efficient mesh-based feature embedding that takes advantage of consistent topology for the hand mesh, as presented in Fig.~\ref{fig:emb}. By providing a condition of personalized hand mesh $\mathcal{M}$ and an event with pose $\theta_t$ at a certain time $t$, our feature embedding module generates mesh features $f_t$ with respect to the $t$ moment as follows \begin{equation}
    f_t = E(p_t | \bar{f}_\mathcal{M}),
\end{equation} where $p_t$ denotes the event at $t$ moment. $\bar{f}_\mathcal{M}$ represents the average features of the hand mesh. 
It is challenging for multi-layer perceptrons (MLPs) to discern the influence of specific conditions on mesh features, leading to divergence in results. To disentangle the effects of conditions and events on mesh features, we design the following embedding function
\begin{equation}
    E(p_t | \bar{f}_\mathcal{M}) = \bar{f}_\mathcal{M} + e(p_t, Q) * \mathcal{K},
\end{equation} where $Q$ is vertex latent code to encode different vertices. $p_t$ is querying events, and $e$ denotes the event decoder of vertex features with MLPs. $\mathcal{K}$ is the code to map events onto features. %The pipeline of the feature embedding is presented in Fig.~\ref{fig:emb}.

The separation of conditions and events enables the interpretable acquisition of personalized hand features $f_t$ under the event $p_t$. Moreover, the feature embedding demonstrates faster convergence and improved accuracy with the constraint of average features $\bar{f}_\mathcal{M}$. In our proposed XHand model, the event $p_t$ represents the pose $\theta_t$ at the $t$ moment. Feature embeddings $E_{lbs}$, $E_{D}$ and $E_{\rho}$ with their corresponding latent code $Q_{lbs}$, $Q_D$ and $Q_\rho$ make use of the same structure of $E(\theta_t | \bar{f}_\mathcal{M})$ except that the predicted mesh features $f_t$ are different.

\noindent\textbf{Inverse Rendering.} In order to train the three feature embeddings $E_D$, $E_{lbs}$ and $E_{\rho}$ simultaneously, an inverse renderer is employed to render images. Assuming that the skin color follows the Lambertian reflectance model~\cite{sfs}, the renderer $B$ can be obtained by calculating the illumination matrix $\mathbf{G}$, the vertex normal $\mathcal{N}$, and the vertex albedo $\rho$ using the following equations \begin{equation}\label{eq:render}
    B(\pi^i) = \rho\cdot SH(\mathbf{G}, \mathcal{N}),
\end{equation} where $\pi^i$ is camera parameters of $i$-th viewpoint. $SH(\cdot)$ represents sphere harmonic (SH) function of the third order. Therefore, we can effectively utilize the geometric and albedo of the mesh to achieve rapid and differentiable rendering.

\noindent\textbf{Mesh-based Neural Rendering.}
 The neural implicit representation-based methods usually employ volume rendering along its corresponding camera ray $\mathbf{d}$ to acquire pixel color. Instead, we employ a mesh-based neural rendering method to render photo-realistic image by taking advantage of geometric alignment of the mesh. % This method leverages the preserved topology of our refined hand representation, resulting in enhanced visual fidelity. 

Mesh is explicitly represented by triangular facets so that the intersection points between rays and meshes are located within the facets. The positional and feature vector information that describe meshes are bound to their vertices.
Therefore, the attributes of intersection points are calculated by interpolating the three vertices of triangular facet to its intersection point. The efficient differentiable rasterization~\cite{Laine2020diffrast} ensures the feasibility of inverse rendering and mesh-based neural rendering.

Given a camera view $(\pi^i)$, our proposed mesh-based neural rendering $\mathcal{C}(\pi^i)$ is calculated with points position $\mathbf{x}$, feature vector $\mathbf{h}$, surface normal $\mathbf{n}$ and ray direction $\mathbf{d}$ \begin{equation}
    \mathcal{C}(\pi^i) = c(\mathbf{x}, \mathbf{n}, \mathbf{h}, \mathbf{d}),
\end{equation} 
where $\mathbf{x}$, $\mathbf{h}$ and $\mathbf{n}$ are obtained through interpolation with $\mathcal{M}_{fine}$. $\mathbf{h}$ contains latent codes $Q_D$ and $Q_\rho$ detached from $E_D$ and $E_\rho$, and rendering latent codes $Q_{render}$.

\subsection{Training Process}
\label{sec:training}

As mentioned above, we need to learn the parameters of three feature embeddings $E_D$, $E_{lbs}$ and $E_{\rho}$ and the neural renderer $\mathcal{C}$, utilizing the multi-view image sequence.

To train XHand model, the average features $\bar{f}_\mathcal{M}$ of mesh in feature embedding significantly affect training efficiency and results. Random initialization greatly impact training due to estimation errors in $E_{lbs}$ and $E_D$,  which may lead to the failure of inverse rendering. Therefore, it is crucial to initialize the neural hand representation. To this end, we employ the reconstruction result of the first frame ($t=1$) as the initial model for the successive frames. For each subsequent frame, we minimize the following objective in training\begin{equation}
    \mathcal{L} = \mathcal{L}_{RGB} + \mathcal{L}_{reg},
\end{equation} where $\mathcal{L}_{RGB}$ represents the rendering loss. $\mathcal{L}_{reg}$ is the regularization term. To emphasize skin wrinkles while constraining the degree of vertex variation, we suggest a part-aware Laplace smoothing term $\mathcal{L}_{reg}$.

\noindent\textbf{Initialization of XHand.} Inspired by~\cite{bib:nccsfs}, we initialize XHand model from multi-view images at the moment $t=1$ and predict the lighting coefficients $\mathbf{G}$ for each viewpoint. Then, we jointly optimize the point cloud and albedo through inverse rendering. Mesh generation is obtained from Eq.~\ref{eq:mesh}, and the rendering equation is derived from Eq.~\ref{eq:render}, where the vertex normal $\mathcal{N}$ is computed from the mesh vertices. The optimization targets are vertex displacement $D$ and vertex albedo $\rho$, following the energy equation below \begin{equation}
    \mathcal{L}_{init} = \sum|B(\pi^i) - I_i| + \sum L * D + \sum L * \rho,
\end{equation} where $\sum|\cdot|$ denotes L1 error and $L$ is the Laplacian matrix. Laplacian smoothing terms $L * D$ and $L * \rho$ are employed to constrain the optimization. The obtained $D$ and $\rho$ are used as the initialization for $E_D$ and $E_\rho$. The initialization of $E_{lbs}$ is obtained from MANO~\cite{MANO}.

\noindent\textbf{Loss Functions of XHand.}
Our loss function mainly consists of two parts: rendering loss $\mathcal{L}_{RGB}$ and regularization loss $\mathcal{L}_{reg}$. In terms of $\mathcal{L}_{RGB}$, inspired by Kerbl et al.~\cite{kerbl20233d}, we use L1 error combined with a D-SSIM term \begin{equation} \begin{aligned}
    \mathcal{L}_{RGB} &= \mathcal{L}_{inv} + \mathcal{L}_{neu} \\ &= \lambda_1\sum|B(\pi^i) - I_i| + (1-\lambda_1)\mathcal{L}_{SSIM}(B(\pi^i), I_i) \\ &+ \lambda_2\sum|\mathcal{C}(\pi^i) - I_i| + (1-\lambda_2)\mathcal{L}_{SSIM}(\mathcal{C}(\pi^i), I_i),
\end{aligned}\end{equation} where $\lambda$ denotes balanced weights. $\mathcal{L}_{inv}$ is used to minimize the loss of inverse rendering, optimizing the parameters of feature embeddings. $\mathcal{L}_{neu}$ minimizes the error of mesh-based neural rendering.%, while the latent code of the feature embeddings is detached, preventing the gradient from propagating forward.

To enhance the efficiency of extracting geometric information from images, the part-aware Laplace smoothing $\mathcal{L}_{p-lap}$ is introduced. The Laplace smooth matrix $\mathbf{A}$ of mesh feature $f$ is defined as follows\begin{equation}
\mathbf{A} = L * f.
\end{equation} Hierarchical weights $\phi_{p-lap}$ are introduced to balance the weights of features with different levels of smoothness. $\varphi_{i}$ in matrix $\phi_{p-lap}$ are defined as follows \begin{equation}
\varphi_{i} = \left\{\begin{array}{l} \lambda_{p_1} \quad 0 < \mathbf{A}_{i} < p_1 
\\ \lambda_{p_2} \quad p_1 < \mathbf{A}_{i} < p_2
\\ ...
\end{array}\right.
,
\end{equation} where $p$ represents the threshold values for the hierarchical weighting. The part-aware Laplace smoothing $\mathcal{L}_{p-lap}$ is used to reduce excessive roughness in albedo and displacement without affecting the fine details, defined as follows \begin{equation}
    \mathcal{L}_{p-lap}(f) = \sum \phi_{p-lap}\mathbf{A}.
\end{equation} 

To ensure the smoothness of optimized vertices and vertex albedo, we introduce the following regularization term $\mathcal{L}_{reg}$ for conforming to the geometric characteristics of the hand\begin{equation} \begin{aligned}
\mathcal{L}_{reg} &= \mathcal{L}_{p-lap}(\rho) + \mathcal{L}_{p-lap}(D) \\ & + \lambda_{3}\mathcal{L}_{mask} + \lambda_{4}\mathcal{L}_{e} + \lambda_{5}\mathcal{L}_{d}.\label{eq:eq1}
\end{aligned}\end{equation} Each term is assigned with a constant coefficient denoted by $\lambda$. $\mathcal{L}_{mask}$ represents the $L_1$ loss between the rendered mask $\hat{M}$ and the original MANO mask $M_{MANO}$, defined as \begin{equation}
    \mathcal{L}_{mask} = \sum|\hat{M} - M_{MANO}|.
\end{equation} 
$\mathcal{L}_{e}$, $\mathcal{L}_{d}$ are defined as\begin{equation}
    \mathcal{L}_{e} = \sum\limits_{i,j}||E_{ij}||^2,
    \end{equation} \begin{equation}
    \mathcal{L}_{d} = \sum||D||^2,
\end{equation} where $E_{ij}$ is obtained by calculating the Euclidean distance $||\cdot||^2$ between adjacent vertices $V_i$ and $V_j$ on the mesh edges. $\mathcal{L}_{e}$ is used to restrict the length of $E_{ij}$. $\mathcal{L}_{e}$ and $\mathcal{L}_{d}$ are utilized to ensure that the optimized hand remains close to the MANO model.
